Graph Relation Distillation for Efficient Biomedical Instance Segmentation

Instance-aware embeddings predicted by deep neural networks have revolutionized biomedical instance segmentation, but its resource requirements are substantial. Knowledge distillation offers a solution by transferring distilled knowledge from heavy teacher networks to lightweight yet high-performance student networks. However, existing knowledge distillation methods struggle to extract knowledge for distinguishing instances and overlook global relation information. To address these challenges, we propose a graph relation distillation approach for efficient biomedical instance segmentation, which considers three essential types of knowledge: instance-level features, instance relations, and pixel-level boundaries. We introduce two graph distillation schemes deployed at both the intra-image level and the inter-image level: instance graph distillation (IGD) and affinity graph distillation (AGD). IGD constructs a graph representing instance features and relations, transferring these two types of knowledge by enforcing instance graph consistency. AGD constructs an affinity graph representing pixel relations to capture structured knowledge of instance boundaries, transferring boundary-related knowledge by ensuring pixel affinity consistency. Experimental results on a number of biomedical datasets validate the effectiveness of our approach, enabling student models with less than $ 1\%$ parameters and less than $10\%$ inference time while achieving promising performance compared to teacher models.

==> parts/algo.tex <==


\begin{algorithm}[t]
    \footnotesize
     \SetAlgoLined
     \SetAlgoShortEnd
     
     \SetKw{KwInput}{Input:}
     \SetKw{KwOutput}{Output:}
     \SetKw{KwPreprocess}{Preprocessing:}
     \SetKw{KwInit}{Initialization:}
     
     \KwInput Corrupted image $S$ and a binary mask, reference image $R$
    
     \KwOutput Completed image $T$
    
     \KwPreprocess Extract feature pyramids $\{F^L_S\}^5_{L=1}$, $\{F^L_R\}^5_{L=1}$ by a feed-forward of $S$, $R$ through the VGG19 network
    
     \KwInit For the deepest layer, initialize NNF $\phi_{S \rightarrow R}^{5}$, $\phi_{R \rightarrow S}^{5}$ as identity mapping, $C^5_S=F^5_S$ and $C^5_R=F^5_R$
     
     \For{$L=5 \text{ to } 1$}
     {
     Build NNF: map $C^L_S$ to $C^L_R$ to obtain $\phi_{S \rightarrow R}^{L}$, map $C^L_R$ to $C^L_S$ to obtain $\phi_{R \rightarrow S}^{L}$
    
     Find mutual NNs, pick the set of reliable anchors $\hat{B}$ around the mask
    
     \For{$b \in \hat{B}$}
     {
     Interpolate NNF in its local region $G^L_b$ to get $\phi_{S \rightarrow R}^{L} \left[ G_{b}^{L}\right]$
     }
    
     Aggregate interpolated NNF $\hat{\phi}^{L}_{S \rightarrow R}$ with function $f$ and $\left\{\hat{\phi}_{S \rightarrow R}^{L} \left[ G_{b}^{L} \right], b \in \hat{B}\right\}$ (Eq.~\ref{eq:agg})
    
     \If{$L>1$}
     {
     Estimate $H_{S}^{L-1}$, $H_{R}^{L-1}$ with aligned features $\tilde{F}_{S}^{L}$, $\tilde{F}_{R}^{L}$ and $\mathrm{VGG}_{L-1}^{L}\left( \cdot \right)$
    
     Obtain next layer common features $C_{S}^{L-1}$, $C_{R}^{L-1}$ using Eq.~\ref{eq:common}
    
     Upsample $\phi_{S \rightarrow R}^{L}$ to $\phi_{S \rightarrow R}^{L-1}$, $\phi_{R \rightarrow S}^{L}$ to $\phi_{R \rightarrow S}^{L-1}$
     }
     }
     Set $\phi_{R \rightarrow S} = \phi_{R \rightarrow S}^{1}$, $\hat{\phi}_{S \rightarrow R} = \hat{\phi}_{S \rightarrow R}^{1}$
    
     Warp $S_{warp}$ with $S$ and $\phi_{R \rightarrow S}$, warp $T$ with $S_{warp}$ and $\hat{\phi}_{S \rightarrow R}$
    \caption{Reference-guided Inpainting via Deep Feature Matching}
    \label{algo:refmatch}
    \end{algorithm}

==> parts/table_1.tex <==

\begin{table*}[ht]
    % Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
    % \small
    \caption{\textbf{Quantitative comparison with baselines.} Our approach consistently improve the perfromance of non-reference methods, especially in terms of both nonbline and blind perception metrics. Ours (M) denotes using method M as the initialization method for our approach.} %since we do not optimize the pixel-level fidelity like learning-based methods  both non-reference and reference-guided.}
    \renewcommand{\arraystretch}{1.4}
    % \begin{center}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{c|cccc|cc|cccc|cc}
        \hline
        Dataset                               & \multicolumn{6}{c|}{image matching challenge}                                                                                                                 & \multicolumn{6}{c}{ukbench}                                                                                                                                                     \\ \hline
        Metric                                & \multicolumn{4}{c|}{Perceptual}                                                                                        & \multicolumn{2}{c|}{Distortion}   & \multicolumn{4}{c|}{Perceptual}                                                                                                             & \multicolumn{2}{c}{Distortion}    \\ \hline
        w/o ref.                              & LPIPS $\downarrow$ & FID $\downarrow$ & NIQE $\downarrow$                     & BRISQUE $\downarrow$                   & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & FID $\downarrow$ & NIQE $\downarrow$                     & \multicolumn{1}{c|}{BRISQUE $\downarrow$}                   & PSNR $\uparrow$ & SSIM $\uparrow$ \\ \hline
        cv.inpaint                            & 0.0159             & 5.98             & \cellcolor[HTML]{EFEFEF}5.38                                  & \cellcolor[HTML]{EFEFEF}26.43                                  & 33.56           & 0.9860          & 0.0227             & 25.57            & \cellcolor[HTML]{EFEFEF}5.58                                  & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}27.28}                                  & 31.51           & 0.9843          \\
        PatchMach                             & 0.0186             & 6.63             & \cellcolor[HTML]{EFEFEF}5.41          & \cellcolor[HTML]{EFEFEF}26.59          & 31.94           & 0.9844          & 0.0293             & 30.92            & \cellcolor[HTML]{EFEFEF}5.61          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}27.44}          & 30.47           & 0.9829          \\
        EdgeCnt                               & 0.0156             & 5.52             & \cellcolor[HTML]{EFEFEF}5.33          & \cellcolor[HTML]{EFEFEF}26.39          & 34.01           & 0.9868          & 0.0221             & 23.68            & \cellcolor[HTML]{EFEFEF}5.52          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}27.24}          & 32.23           & 0.9848          \\
        MEDFE                                 & 0.0163             & 5.82             & \cellcolor[HTML]{EFEFEF}5.30          & \cellcolor[HTML]{EFEFEF}26.45          & 33.40           & 0.9858          & 0.0240             & 26.82            & \cellcolor[HTML]{EFEFEF}5.41          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}27.27}          & 31.92           & 0.9835          \\ \hline
        w/ ref.                               & LPIPS $\downarrow$ & FID $\downarrow$ & NIQE $\downarrow$                     & BRISQUE $\downarrow$                   & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & FID $\downarrow$ & NIQE $\downarrow$                     & \multicolumn{1}{c|}{BRISQUE $\downarrow$}                   & PSNR $\uparrow$ & SSIM $\uparrow$ \\ \hline
        SC                                    & 0.0591             & 12.66            & \cellcolor[HTML]{EFEFEF}5.33          & \cellcolor[HTML]{EFEFEF}26.45          & 24.99           & 0.9291          & 0.0394             & 34.91            & \cellcolor[HTML]{EFEFEF}5.52          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}27.26}          & 27.02           & 0.9658          \\
        PRINCE                                & 0.0314             & 9.43             & \cellcolor[HTML]{EFEFEF}5.40          & \cellcolor[HTML]{EFEFEF}26.48          & 30.97           & 0.9823          & 0.0360             & 24.06            & \cellcolor[HTML]{EFEFEF}5.47          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}27.36}          & 29.51           & 0.9823          \\
        Ours (cv.inpaint)                      & 0.0134             & 4.58             & \cellcolor[HTML]{EFEFEF}5.25          & \cellcolor[HTML]{EFEFEF}26.06          & 34.02           & 0.9862          & 0.0189             & 20.18            & \cellcolor[HTML]{EFEFEF}5.43          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}26.93}          & 32.13           & \textbf{0.9854} \\
        \multicolumn{1}{l|}{Ours (PatchMatch)} & 0.0137             & 4.74             & \cellcolor[HTML]{EFEFEF}5.26          & \cellcolor[HTML]{EFEFEF}\textbf{25.95} & 33.28           & 0.9848          & 0.0193             & 20.26            & \cellcolor[HTML]{EFEFEF}\textbf{5.40} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{26.78}} & 32.46           & 0.9831          \\
        EdgeCnt+                              & 0.0156             & 5.48             & \cellcolor[HTML]{EFEFEF}5.32          & \cellcolor[HTML]{EFEFEF}26.38          & 33.80           & \textbf{0.9869} & 0.0218             & 23.27            & \cellcolor[HTML]{EFEFEF}5.50          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}27.23}          & 32.36           & 0.9845          \\
        Ours (EdgeCnt)                         & \textbf{0.0133}    & \textbf{4.49}    & \cellcolor[HTML]{EFEFEF}5.25          & \cellcolor[HTML]{EFEFEF}26.04          & \textbf{34.49}  & \textbf{0.9869} & 0.0184             & \textbf{19.31}   & \cellcolor[HTML]{EFEFEF}5.43          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}26.97}          & \textbf{32.92}  & 0.9853          \\
        MEDFE+                                & 0.0162             & 5.80             & \cellcolor[HTML]{EFEFEF}5.30          & \cellcolor[HTML]{EFEFEF}26.40          & 33.41           & 0.9859          & 0.0240             & 26.59            & \cellcolor[HTML]{EFEFEF}5.41          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}27.28}          & 31.93           & 0.9836          \\
        Ours (MEDFE)                           & 0.0138             & 4.75             & \cellcolor[HTML]{EFEFEF}\textbf{5.24} & \cellcolor[HTML]{EFEFEF}26.11          & 34.01           & 0.9860          & \textbf{0.0182}    & 21.05            & \cellcolor[HTML]{EFEFEF}5.41          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}26.96}          & 32.85           & 0.9836          \\ \hline
        \end{tabular}%
        }
    % \end{center}
    \label{table:result}
    \end{table*}
    

==> parts/table_2.tex <==

\begin{table*}[h]    

    \caption{\textbf{Ablation study on the structure-aware progressive interpolation.} Compared with without correction strategy and the two alternative strategies RoI interp. and Corner interp., our strategy of picking mutual NNs as reliable anchors and then interpolating mismatched mapping vectors progressively estimates smooth and reasonable estimation, and thus produces better completed results. }
    \renewcommand{\arraystretch}{1.4}
    % \setlength{\arrayrulewidth}{1pt}
    % \begin{center}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{c|cc|cc|cc|cccccc}
    \hline
    Dataset                  & \multicolumn{6}{c|}{image matching challenge}                                                                                             & \multicolumn{6}{c}{ukbench}                                                                                                                                                       \\ \hline
                             & \multicolumn{2}{c|}{Mapping Error} & \multicolumn{2}{c|}{Perceptual}                                & \multicolumn{2}{c|}{Distortion}   & \multicolumn{2}{c|}{Mapping Error}                      & \multicolumn{2}{c|}{Perceptual}                                                     & \multicolumn{2}{c}{Distortion}    \\ \cline{2-13} 
    \multirow{-2}{*}{Metric} & EPE $\downarrow$ & F1 $\downarrow$ & LPIPS $\downarrow$             & FID $\downarrow$             & PSNR $\uparrow$ & SSIM $\uparrow$ & EPE $\downarrow$ & \multicolumn{1}{c|}{F1 $\downarrow$} & LPIPS $\downarrow$             & \multicolumn{1}{c|}{FID $\downarrow$}              & PSNR $\uparrow$ & SSIM $\uparrow$ \\ \hline
	w/o correction              & 20.28            & 43.46\%         & 0.0179 & 6.72 & 31.36           & 0.9815          & 22.61            & \multicolumn{1}{c|}{51.03\%}         & 0.0269 & \multicolumn{1}{c|}{28.09} & 29.43           & 0.9783          \\
    RoI interp.              & 19.71            & 38.89\%         & \cellcolor[HTML]{FFFFFF}0.0176 & \cellcolor[HTML]{FFFFFF}6.49 & 32.24           & 0.9830          & 21.97            & \multicolumn{1}{c|}{44.53\%}         & \cellcolor[HTML]{FFFFFF}0.0262 & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}26.61} & 30.83           & 0.9805          \\
    Corner interp.           & 20.27            & 40.21\%         & \cellcolor[HTML]{FFFFFF}0.0177 & \cellcolor[HTML]{FFFFFF}6.20 & 32.04           & 0.9824          & 22.61            & \multicolumn{1}{c|}{45.25\%}         & \cellcolor[HTML]{FFFFFF}0.0256 & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}27.95} & 30.78           & 0.9802          \\
    Structure-aware interp.  & \textbf{14.59}            & \textbf{25.77\%}         & \cellcolor[HTML]{FFFFFF}\textbf{0.0137} & \cellcolor[HTML]{FFFFFF}\textbf{4.74} & \textbf{33.28}           & \textbf{0.9848}          & \textbf{17.79}            & \multicolumn{1}{c|}{\textbf{33.17\%}}         & \cellcolor[HTML]{FFFFFF}\textbf{0.0193} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{20.26}} & \textbf{32.46}           & \textbf{0.9831}          \\ \hline
    % Upper bound      & -                & -               & \cellcolor[HTML]{FFFFFF}0.0065 & \cellcolor[HTML]{FFFFFF}2.41 & 37.99           & 0.9928          & -                & \multicolumn{1}{c|}{-}               & \cellcolor[HTML]{FFFFFF}0.0095 & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}10.18} & 36.82           & 0.9915          \\ \hline
    \end{tabular}
    }
    % \end{center}
    \label{table:ablation}
    \end{table*}

==> parts/table_3.tex <==

\begin{table*}[h]
    % Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
    % \small
    \caption{\textbf{Ablation experiments without initial estimation.} There are clear improvements in performance after applying our approach on both types of images without the initial estimation.} %since we do not optimize the pixel-level fidelity like learning-based methods  both non-reference and reference-guided.}
    \renewcommand{\arraystretch}{1.4}
    % \begin{center}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{c|cccc|cc|cccc|cc}
        \hline
        Dataset                               & \multicolumn{6}{c|}{image matching challenge}                                                                                                                 & \multicolumn{6}{c}{ukbench}                                                                                                                                                     \\ \hline                                & \multicolumn{4}{c|}{Perceptual}                                                                                        & \multicolumn{2}{c|}{Distortion}   & \multicolumn{4}{c|}{Perceptual}                                                                                                             & \multicolumn{2}{c}{Distortion}    \\ \cline{2-13} 
        \multirow{-2}{*}{Metric}                          & LPIPS $\downarrow$ & FID $\downarrow$ & NIQE $\downarrow$                     & BRISQUE $\downarrow$                   & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & FID $\downarrow$ & NIQE $\downarrow$                     & \multicolumn{1}{c|}{BRISQUE $\downarrow$}                   & PSNR $\uparrow$ & SSIM $\uparrow$ \\ \hline
        Fill Gray Color                             & 0.0334             & 9.66             & \cellcolor[HTML]{EFEFEF}5.54          & \cellcolor[HTML]{EFEFEF}27.18          & 30.22           & 0.9809          & 0.0387             & 33.89            & \cellcolor[HTML]{EFEFEF}5.58          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}28.97}          & 29.37           & 0.9789          \\
        
        Ours (Gray Color)                      & 0.0176             & 5.76             & \cellcolor[HTML]{EFEFEF}5.28          & \cellcolor[HTML]{EFEFEF}26.08          & 32.15           & 0.9825          & 0.0239             & 25.46            & \cellcolor[HTML]{EFEFEF}5.40          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}26.84}          & 30.71           & 0.9798 \\
        Paste Random Patch                               & 0.0237             & 7.51             & \cellcolor[HTML]{EFEFEF}5.45          & \cellcolor[HTML]{EFEFEF}26.66          & 29.85           & 0.9800          & 0.0364             & 33.40            & \cellcolor[HTML]{EFEFEF}5.57          & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}27.39}          & 27.97           & 0.9784          \\
        \multicolumn{1}{l|}{Ours (Random Patch)} & 0.0164             & 5.57             & \cellcolor[HTML]{EFEFEF}5.44          & \cellcolor[HTML]{EFEFEF}26.11 & 32.26           & 0.9834          & 0.0263             & 27.17            & \cellcolor[HTML]{EFEFEF}5.39 & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}26.86} & 30.48           & 0.9811          \\ \hline
        \end{tabular}%
        }
    % \end{center}
    \label{table:woinit}
    \end{table*}
